FREST: Feature RESToration for Semantic Segmentation under Multiple Adverse Conditions

Robust semantic segmentation under adverse conditions is crucial in real-world applications. To address this challenging task in practical scenarios where labeled normal condition images are not accessible in training, we propose FREST, a novel feature restoration framework for source-free domain adaptation (SFDA) of semantic segmentation to adverse conditions. FREST alternates two steps: (1) learning the condition embedding space that only separates the condition information from the features and (2) restoring features of adverse condition images on the learned condition embedding space. By alternating these two steps, FREST gradually restores features where the effect of adverse conditions is reduced. FREST achieved a state of the art on two public benchmarks (i.e., ACDC and RobotCar) for SFDA to adverse conditions. Moreover, it shows superior generalization ability on unseen datasets.

==> Figures/detailed_structure.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-4mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \vspace{-3mm}
%     \label{fig:detail}
% \end{figure}


% \begin{figure}[t!]

% \centering

\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{wrapfigure}{br}{0.36\linewidth}
  \centering
  % \vspace{-7mm}
  \begin{minipage}{1.0\linewidth}
        \centering
        \includegraphics[width=0.9\textwidth]{Figures/pdf/detail_module.pdf}
        % \vspace{-3mm}
    \caption{
    % Detailed structure of our network computing $\textbf{c}^l$ and $\textbf{f}^l$.
    Detail of the encoder with the condition strainer.
    % the encoder with the condition strainer.
    % our network computing condition-infused feature $\textbf{c}^l$.
    Condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
    % (b) The encoder without the strainer produces the restored feature $\textbf{f}^l$ used for inference at the $l$-th layer.
    }
    \label{fig:detail}
  \end{minipage}
  % \vspace{-6mm}
\end{wrapfigure}

% \begin{minipage}{0.47\linewidth}
% \centering   
% \includegraphics[width=0.94\textwidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-3mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \label{fig:detail}
% \end{minipage}
% \hspace{2mm}
% % \end{figure}
% % \vspace{-1mm}

==> Figures/loss_dis.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-4mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \vspace{-3mm}
%     \label{fig:detail}
% \end{figure}


% \begin{figure}[t!]

% \centering
\begin{wrapfigure}{br}{0.375\linewidth}
  \centering
  \vspace{-7.5mm}
  \begin{minipage}{1.0\linewidth}
        \centering
        \includegraphics[width=0.9\textwidth]{Figures/pdf/dis_loss.pdf}
        \vspace{-3mm}
    \caption{Detail of the adverse condition discriminator.
    }
    \vspace{-12mm}
    \label{fig:loss_dis}
  \end{minipage}
  % \vspace{-9mm}
\end{wrapfigure}

% \begin{minipage}{0.47\linewidth}
% \centering   
% \includegraphics[width=0.94\textwidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-3mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \label{fig:detail}
% \end{minipage}
% \hspace{2mm}
% % \end{figure}
% % \vspace{-1mm}

==> Figures/overall_architecture.tex <==

\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{figure*}[t]
    \centering
    % \vspace{0mm}
    \includegraphics[width=1\linewidth]{Figures/pdf/overall_architecture_v4.pdf}
    % \vspace{-4mm}
    \caption{
    The overall architecture and training strategy.
    The segmentation network is pre-trained using a labeled source dataset.
    % , with no further access to this dataset.
    % The encoder $\phi_\textrm{enc}$ and decoder $\phi_\textrm{dec}$ of the segmentation network are initialized with pre-trained parameters from a labeled source dataset., with no further access to this dataset. 
    For each iteration, the condition strainer and segmentation network are trained alternatingly.
    The frozen modules are shown in gray, the trainable modules are highlighted in red, and ``sg'' denotes the stop gradient.
    % The exponential moving average (EMA) model is represented by dashed lines, the frozen models are shown in gray, and the trainable models are highlighted in red.
    (\textit{Step 1}) The condition strainer and projection head are trained to learn the condition embedding space.
    (\textit{Step 2}) The segmentation network is trained to restore features from adverse to normal conditions on the condition embedding space.
    % (\textit{Step 2}) The segmentation network is trained using the standard entropy minimization $\mathcal{L}_\textrm{ent}$ and self-training loss $\mathcal{L}_\textrm{self}$, alongside $\mathcal{L}_\textrm{mimic}$ and $\mathcal{L}_\textrm{dis}$ for restoring features from adverse to normal conditions.
    For evaluation, only the encoder $\phi_\textrm{enc}$ and decoder $\phi_\textrm{dec}$ of the segmentation network are utilized.
    }
    % \vspace{-1mm}
\label{fig:pipeline}
\end{figure*}



==> Figures/pos_and_dis.tex <==
\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{figure}[t!]
\centering
  \begin{minipage}{0.56\linewidth}
        \includegraphics[width=0.98\textwidth]{Figures/pdf/pos_select.pdf}
        % \vspace{-1mm}
    \caption{
    Detail of positive embedding sampling strategy in the condition-specific learning.
    }
    % \vspace{-6mm}
    \label{fig:pos_select}
  \end{minipage}
  % \hspace{1mm}
  \quad % ----------------------------------
  \begin{minipage}{0.34\linewidth}
        \centering
        \includegraphics[width=0.8\textwidth]{Figures/pdf/dis_loss.pdf}
        % \vspace{-1mm}
    \caption{Detail of the adverse condition discriminator.
    }
    % \vspace{-6mm}
    \label{fig:loss_dis}
  \end{minipage}
% \vspace{-1mm}
\end{figure}

==> Figures/pos_select.tex <==
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-4mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \vspace{-3mm}
%     \label{fig:detail}
% \end{figure}


% \begin{figure}[t!]

% \centering
\begin{wrapfigure}{br}{0.5\linewidth}
  \centering
  \vspace{-6mm}
  \begin{minipage}{1.0\linewidth}
        \includegraphics[width=1\textwidth]{Figures/pdf/pos_select.pdf}
        \vspace{-3mm}
    \caption{
    Detail of positive embedding sampling strategy.
    }
    \vspace{-6mm}
    \label{fig:pos_select}
  \end{minipage}
  % \vspace{-9mm}
\end{wrapfigure}

% \begin{minipage}{0.47\linewidth}
% \centering   
% \includegraphics[width=0.94\textwidth]{Figures/pdf/detail_module.pdf}
%     \vspace{-3mm}
%     \caption{
%     Detailed structure of our network where feature $\textbf{c}^l$ and $\textbf{f}^l$ are computed.
%     (a) The condition strainers are connected to the original feed-forward layer (FFN) and multi-head self-attention layer (MHSA) through the residual connections.
%     (b) The encoder $\phi_{\mathrm{enc}}$ at the $l$-th layer produces the feature $\textbf{f}^l$ used for feature restoration and inference process.
%     }
%     \label{fig:detail}
% \end{minipage}
% \hspace{2mm}
% % \end{figure}
% % \vspace{-1mm}

==> Figures/qualitative.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/pdf/qualitative_results.pdf}
    % \vspace{-5mm}
    \caption{
    Qualitative results of FREST (Ours), its baseline (SegFormer~\cite{xie2021segformer}), and CMA~\cite{bruggemann2023contrastive} on ACDC and RobotCar.
    }
\label{fig:qual_main}
% \vspaceBottomFigure
% \vspace{-1mm}
\end{figure*}



==> Figures/teaser.tex <==
% \setlength{\floatsep}{3pt plus 3pt minus 10pt}
% \setlength{\textfloatsep}{8pt plus 3pt minus 5pt}
\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/pdf/teaser_v2.pdf}
    % \vspace{-6mm}
    \caption{
    (a) The setting of SFDA to adverse conditions. 
    A segmentation model, initially pre-trained on a labeled source dataset, is adapted to adverse conditions using pairs of unlabeled adverse and normal images.
    (b) Following the SFDA setting, FREST restores features of adverse condition images to simulate the normal condition. 
    }
    % \vspace{-1mm}
    \label{fig:teaser}
\end{figure}

==> Tables/comp_ablation_component.tex <==
\begin{table}[t!]
\centering
  \begin{minipage}{0.43\linewidth}
    \caption{
    Loss analysis on (a) Step 1 and (b) Step 2. %on ACDC \textit{val} set.
    }
  \renewcommand{\arraystretch}{1.1}
    \centering
    \begin{subtable}[h]{0.45\linewidth}
    \scalebox{0.92}{
    \begin{tabular}{@{}ccc@{}}\toprule
     $\mathcal{L}_\textrm{self}$     &  	 $\mathcal{L}_\textrm{spec}$  & mIoU \\ 
    \midrule
      &  &    64.3    \\
     \checkmark &  &   64.8  \\
     \checkmark & \checkmark  &  \textbf{68.6}       \\
    \bottomrule
    \end{tabular}
    }
    \caption{}
    \end{subtable}
    \begin{subtable}[h]{0.45\linewidth}
    \scalebox{0.92}{
    \begin{tabular}{@{}ccc@{}}\toprule
    $\mathcal{L}_\textrm{resto}$   &  $\mathcal{L}_\textrm{dis}$ & mIoU \\ 
    \midrule
           &    &   62.7  \\
          \checkmark &    &   67.2   \\
          \checkmark &  \checkmark   &       \textbf{68.6} \\
    \bottomrule
    \end{tabular}
    }
    \caption{}
    \end{subtable}
    \label{tab:abl_loss}
  \end{minipage}
  \quad % ----------------------------------
  \begin{minipage}{0.52\linewidth}
    \centering
    \caption{Analysis of the structure and training strategy in FREST. %on ACDC \textit{val} set.
     }    
  % \renewcommand{\arraystretch}{0.9}
    \scalebox{0.88}{\begin{tabular}{ccccc}
    \toprule
    \multicolumn{2}{c}{Trainable Module } & \multicolumn{2}{c}{Training Strategy}  & \multirow{2}{*}{ mIoU} \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-4}
    Strainer  &  Seg. &  Self-training&FREST  & \\ 
    \midrule
      &  \checkmark    & \checkmark  &    &    62.7    \\
    \checkmark  &  &     \checkmark  &        &   63.1  \\
    \checkmark  &  \checkmark &     \checkmark  &        &   63.2  \\
     \checkmark  &   \checkmark &           & \checkmark & \textbf{68.6} \\
     \bottomrule
    \end{tabular}}
    \label{tab:abl_comp}
  \end{minipage}
\end{table}


==> Tables/comp_ablation_loss.tex <==
\begin{table}
\centering
\begin{subtable}[h]{0.46\linewidth}
\centering
\scalebox{0.9}{
\begin{tabular}{@{}ccc@{}}\toprule
 $\mathcal{L}_\textrm{self}$     &  	 $\mathcal{L}_\textrm{spec}$  & mIoU \\ 
\midrule
  &  &    64.3    \\
 \checkmark &  &   64.8  \\
 \checkmark & \checkmark  &  \textbf{68.6}       \\
\bottomrule
\end{tabular}
}
\caption{}
\end{subtable}
\begin{subtable}[h]{0.46\linewidth}
\centering
\scalebox{0.9}{
\begin{tabular}{@{}ccc@{}}\toprule
$\mathcal{L}_\textrm{mimic}$   &  $\mathcal{L}_\textrm{dis}$ & mIoU \\ 
\midrule
       &    &   62.7  \\
      \checkmark &    &   67.2   \\
      \checkmark &  \checkmark   &       \textbf{68.6} \\
\bottomrule
\end{tabular}
}
\caption{}
\end{subtable}
\vspace{-2mm}
\caption{
Loss analysis on ACDC \textit{val} set. (a) Losses for learning condition-specific information and (b) Losses for learning segmentation network using feature restoration.
}
\vspace{-3mm}
\label{tab:abl_loss}
\end{table}







% \begin{table}[!t]
%     \centering
%     \renewcommand{\arraystretch}{1.0}
%     \scalebox{1.0}{\begin{tabular}{ccc}
%     \toprule
%     Loss &   & mIoU \\
%     \midrule
%     \multicolumn{3}{c}{\textbf{Stage 1}} \\
%     \midrule
%      $\mathcal{L}_\textrm{self}$     &  	 $\mathcal{L}_\textrm{specific}$       \\
%      \checkmark &  &  \textbf{68.6}       \\
%      \checkmark & \checkmark  &  \textbf{68.6}       \\
%     \midrule
%     \multicolumn{3}{c}{\textbf{Stage 2}} \\
%     \midrule
%     $\mathcal{L}_\textrm{reg}$   &  $\mathcal{L}_\textrm{cls}$  & \\
%        &    &     \\
%       \checkmark &    &   67.2   \\
%       \checkmark &  \checkmark   &       \textbf{68.6} \\
%      \bottomrule
%     \end{tabular}}
%     \caption{Analysis of each loss for our framework on the ACDC validation set.
%     }
%     \label{tab:ablation_comp}
%     \vspaceBottomTable
% \end{table}

==> Tables/comp_ablation_loss_backup.tex <==
\begin{table}[!t]
    \centering
    \renewcommand{\arraystretch}{1.0}
    \scalebox{1.0}{\begin{tabular}{lc}
    \toprule
    Loss & mIoU \\
    \midrule
    \multicolumn{2}{c}{\textbf{Stage 1}} \\
    \midrule
     $\mathcal{L}_\textrm{self}$     &  	       \\
     $\mathcal{L}_\textrm{self}$ + $\mathcal{L}_\textrm{specific}$    &  \textbf{68.6}       \\
    \midrule
    \multicolumn{2}{c}{\textbf{Stage 2}} \\
    \midrule
     $\mathcal{L}_\textrm{self}$     &  	       \\
     $\mathcal{L}_\textrm{self}$ + $\mathcal{L}_\textrm{entropy}$     &       \\
     $\mathcal{L}_\textrm{self}$ + $\mathcal{L}_\textrm{entropy}$ + $\mathcal{L}_\textrm{reg}$   &   67.2   \\
     $\mathcal{L}_\textrm{self}$ + $\mathcal{L}_\textrm{entropy}$ + $\mathcal{L}_\textrm{reg}$   + $\mathcal{L}_\textrm{cls}$    &       \textbf{68.6} \\
     \bottomrule
    \end{tabular}}
    % \vspace{-2mm}
    \caption{Analysis of each loss for our framework on the ACDC validation set.
    }
    \label{tab:ablation_comp}
    \vspaceBottomTable
\end{table}

==> Tables/comp_acg.tex <==
% \begin{table}
% \centering%
% \scalebox{0.8}{%
% % \ra{1.3}%
% \begin{tabular}{@{}lccccccccr@{}}\toprule
% \multirow{2}{*}{Method}  && \multicolumn{5}{c}{ACG} & C-Lindau\\
% % \cmidrule{3-7} \cmidrule(lr){2-6} 
% \cmidrule(lr){3-7} \cmidrule(lr){8-8}
% && fog & night & rain & snow & \textbf{all} & normal\\
% % \midrule
% \midrule
% SegFormer~\cite{xie2021segformer}  && 54.0 & 27.9 & 47.5 & 41.2 & 40.1 & \textbf{72.7}\\
% HCL~\cite{huang2021model}  && 54.2 & 28.3 & 48.2 & 42.4 & 40.8 & - \\
% URMA~\cite{fleuret2021uncertainty}  && 54.1 & 31.0 & 51.9 & 45.5 & 44.4 & - \\
% CMA~\cite{bruggemann2023contrastive} && 59.7 & \textbf{40.0} & \underline{59.6} & \textbf{52.2} & \underline{51.3} & 71.8\\
% FREST && \textbf{61.4} & \underline{39.9} & \textbf{61.0} & \underline{51.9} & \textbf{52.6} & \underline{72.5}\\
% \bottomrule
% \end{tabular}
% }%
% % \vspace{-2.5mm}
% \caption{
% Generalization performance of models adapted from Cityscapes to ACDC on ACG and Cityscapes-lindau40 (C-Lindau) in mIoU (\%).
% }%
% \vspace{-3mm}
% \label{tab:comp_acg}
% \end{table}

==> Tables/comp_acg_backup.tex <==
\begin{table}
\centering%
\scalebox{0.9}{%
\ra{1.3}%
\begin{tabular}{@{}lccccccccr@{}}\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{$\mathcal{SF}$} && \multicolumn{5}{c}{ACG mIoU}\\
\cmidrule{4-8} 
&&& fog & night & rain & snow & all \\
% \midrule
% SegFormer~\cite{xie2021segformer} & N/A && 59.4 && 54.0 & 28.0 & 47.7 & 41.4 & 40.2 \\
\midrule
TENT~\cite{wang2021tent} & \checkmark && 52.6 & 27.7 & 47.5 & 41.1 & 40.0 \\
HCL~\cite{huang2021model} & \checkmark && 54.2 & 28.3 & 48.2 & 42.4 & 40.8 \\
URMA~\cite{fleuret2021uncertainty} & \checkmark && 54.1 & 31.0 & 51.9 & 45.5 & 44.4 \\
% \midrule
% DAFormer~\cite{hoyer2022daformer} &&& 52.6 & 21.5 & 47.5 & 33.6 & 40.1 \\
% SePiCo~\cite{xie2023sepico} &&& 53.9 & 20.6 & 46.3 & 36.1 & 38.6 \\
HRDA~\cite{hoyer2022hrda} &&& \underline{60.0} & 27.1 & 56.2 & 43.3 & 48.9 \\
% Refign~\cite{bruggemann2023refign} &&& 72.1 && \\
% \midrule
CMA & \checkmark && 59.7 & \textbf{40.0} & \underline{59.6} & \textbf{52.2} & \underline{51.3} \\
Ours & \checkmark && \textbf{61.4} & \underline{39.9} & \textbf{61.0} & \underline{51.9} & \textbf{52.6} \\
\bottomrule
\end{tabular}
}%
\caption{ACG benchmark generalization performance of models adapted from Cityscapes to ACDC.
$\mathcal{SF}$ denotes a source-free adaptation approach.
}%
\label{tab:comp_acg}
\end{table}

==> Tables/comp_clearweather.tex <==
\begin{table}
\centering%
\scalebox{0.9}{%
\ra{1.3}%
\begin{tabular}{@{}lcr@{}}\toprule
Method & Cityscapes lindau 40 mIoU \\
\midrule
SegFormer~\cite{xie2021segformer} & \textbf{72.7} \\
CMA~\cite{bruggemann2023contrastive} & 71.8 \\
Ours & \underline{72.5} \\
\bottomrule
\end{tabular}
}
\caption{
Results of models adapted from Cityscapes to ACDC on Cityscapes lindau 40 in mIoU (\%).
}%
\label{tab:comp_clearweather}
\end{table}


% \begin{table}
% \centering%
% \scalebox{0.9}{%
% \ra{1.3}%
% \begin{tabular}{@{}lcr@{}}\toprule
% Method & Cityscapes mIoU \\
% \midrule
% SegFormer~\cite{xie2021segformer} & \textbf{82.4} \\
% CMA~\cite{bruggemann2023contrastive} & 81.6 \\
% Ours & \underline{81.7} \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% Results of models adapted from Cityscapes to ACDC on Cityscapes in mIoU (\%).
% }%
% \label{tab:comp_clearweather}
% \end{table}

==> Tables/comp_filter_analysis.tex <==
\begin{table}[t!]
\centering
  \begin{minipage}{0.48\linewidth}
  \centering
  \begin{minipage}{\linewidth}
  \centering
    \caption{The number of parameters for additional modules.
    }
    \renewcommand{\arraystretch}{0.9}
  \scalebox{0.9}{
    \begin{tabular}{lc}
    \toprule
       & Param. \\ \midrule
    SegFormer~\cite{xie2021segformer}       & 81.4M (100\%)\\
    Condition Strainer      &  2.1M (2.6\%)\\
    Projection Layer  &  1.2M (1.5\%)\\ 
    \bottomrule
    \end{tabular}}\label{tab:analy_param}
    \end{minipage}
  \begin{minipage}{\linewidth}
  \centering
    \caption{Impact of restored features $\textbf{f}_\textrm{adv}$.
    }
    \renewcommand{\arraystretch}{0.9}
\scalebox{0.9}{\begin{tabular}{lc}
    \toprule
    Features for Inference & mIoU \\ 
    \midrule
    Condition-infused feature $\textbf{c}_\textrm{adv}$   &  59.0   \\
     Restored feature $\textbf{f}_\textrm{adv}$    &  \textbf{68.6}   \\
     \bottomrule
    \end{tabular}}
    \label{tab:condition_specific_inference}
    \end{minipage}
  \end{minipage}
  \quad % ----------------------------------
  \begin{minipage}{0.48\linewidth}
    \centering
    \caption{
    Performance according to positive embedding selection strategies and loss functions. \textit{Cls.} and \textit{Contra.} denote classification and contrastive loss.
    }
    \renewcommand{\arraystretch}{1.33}
    \scalebox{0.81}{
    \begin{tabular}{l|cc|c}
    \toprule
    Pos. Emb. Selection    & ~\textit{Cls.}~  &  ~\textit{Contra.}~    & ~mIoU~  \\ \midrule
    \multirow{2}{*}{All}           & \checkmark     &                      & 62.9  \\
                                   &                &  \checkmark          & 63.4  \\ \midrule
    (1) $\mathtt{RANDOM}$          &                &  \checkmark          & 62.4 \\
    (2) $\mathtt{LOWEST}$          &                &  \checkmark          &  56.6 \\
    (3) $\mathtt{HIGHEST}$ (Ours)  &                &  \checkmark          &  \textbf{68.6}  \\ 
    \bottomrule
    \end{tabular}
    }
    \label{tab:analy_csl}
  \end{minipage}
\end{table}



==> Tables/comp_robotcar_uda.tex <==

\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{table}[t!]
\centering
  \begin{minipage}{0.23\linewidth}
    \centering
    % \ra{1.2}
    \caption{Comparison with previous methods on City $\to$ RobotCar.
     }    
    % \vspace{-1mm}
     % \vspace{-2mm}
    \scalebox{0.73}{\begin{tabular}{@{}lc@{}}\toprule
    {Method} & mIoU \\ 
    \midrule
    Source model~\cite{xie2021segformer} & 50.0  \\
    HCL~\cite{huang2021model} & 50.1   \\
    URMA~\cite{fleuret2021uncertainty} & 51.6  \\
    URMA + SimT~\cite{guo2022simt} & 52.4  \\
    CMA~\cite{bruggemann2023contrastive} & \underline{54.3}  \\
    % \midrule
    FREST (Ours) & \textbf{58.8} \\
    \bottomrule
    \end{tabular}}
    % \vspace{-2mm}
    \label{tab:comp_robotcar}
  \end{minipage}%
  \quad % ----------------------------------
  \begin{minipage}{0.26\linewidth}
    \centering
    \caption{
    Comparison with UDA methods on City $\to$ ACDC.
    ($\mathcal{SF}$: source-free method).
    }
    % \vspace{-1mm}
    \ra{1.06}
    \scalebox{0.7}{
    \begin{tabular}{@{}lcc@{}}\toprule
    Method & $\mathcal{SF}$ & mIoU \\
    \midrule
    Source model~\cite{xie2021segformer} & & 59.4  \\
    Refign~\cite{bruggemann2023refign} & & 65.5 \\
    HRDA~\cite{hoyer2022hrda} & & 68.0 \\
    HRDA + MIC~\cite{hoyer2023mic}  &  &  \underline{70.4}  \\
    % \midrule
    CMA~\cite{bruggemann2023contrastive} & \checkmark & 69.1 \\
    FREST (Ours) & \checkmark & \textbf{70.7} \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2mm}
    \label{tab:comp_uda}
  \end{minipage}
\quad % ----------------------------------
\begin{minipage}{0.44\linewidth}
    \centering  
    \caption{
    Generalization performance of models adapted from Cityscapes to ACDC on ACG and Cityscapes-lindau40 (C-Lindau).
    }%
    % \vspace{-1mm}
    % \vspace{-2mm}
    \ra{1.08}
    % \ra{1.2}
    \scalebox{0.65}{
    \begin{tabular}{@{}lccccccccr@{}}\toprule
\multirow{2}{*}{Method}  && \multicolumn{5}{c}{ACG} & C-Lindau\\
% \cmidrule{3-7} \cmidrule(lr){2-6} 
\cmidrule(lr){3-7} \cmidrule(lr){8-8}
&& fog & night & rain & snow & \textbf{all} & normal\\
% \midrule
\midrule
SegFormer~\cite{xie2021segformer}  && 54.0 & 27.9 & 47.5 & 41.2 & 40.1 & \textbf{72.7}\\
HCL~\cite{huang2021model}  && 54.2 & 28.3 & 48.2 & 42.4 & 40.8 & - \\
URMA~\cite{fleuret2021uncertainty}  && 54.1 & 31.0 & 51.9 & 45.5 & 44.4 & - \\
CMA~\cite{bruggemann2023contrastive} && 59.7 & \textbf{40.0} & \underline{59.6} & \textbf{52.2} & \underline{51.3} & 71.8\\
FREST (Ours) && \textbf{61.4} & \underline{39.9} & \textbf{61.0} & \underline{51.9} & \textbf{52.6} & \underline{72.5}\\
\bottomrule
\end{tabular}
    }
    % \vspace{-2mm}
% \vspace{-3mm}
\label{tab:comp_acg}
  \end{minipage}
% \vspace{-1mm}
\end{table}

==> Tables/comp_robotcar_uda_backup.tex <==
\begin{table}
\centering
\begin{subtable}[h]{0.194\textwidth}
\centering
\scalebox{0.82}{
\begin{tabular}{@{}lc@{}}\toprule
{Method} & mIoU \\ 
\midrule
Source model & 50.0  \\
% TENT~\cite{wang2021tent}  & 50.1  \\
HCL~\cite{huang2021model} & 50.1   \\
URMA~\cite{fleuret2021uncertainty} & 51.6  \\
URMA + SimT~\cite{guo2022simt} & 52.4  \\
CMA & \underline{54.3}  \\
% \midrule
Ours & \textbf{58.8} \\
\bottomrule
\end{tabular}
}
\caption{}
\end{subtable}
\begin{subtable}[h]{0.278\textwidth}
\centering%
\scalebox{0.95}{
\begin{tabular}{@{}lcc@{}}\toprule
Method & $\mathcal{SF}$ & mIoU \\
\midrule
Refign~\cite{bruggemann2023refign} && 65.5 \\
HRDA~\cite{hoyer2022hrda} && 68.0 \\
HRDA + MIC~\cite{hoyer2023mic}  &  &  \underline{70.4}  \\
% \midrule
CMA & \checkmark & 69.1 \\
Ours & \checkmark & \textbf{70.7} \\
\bottomrule
\end{tabular}
}%
\caption{}
\end{subtable}
\caption{(a) Comparison to the state of the art in model adaptation on Cityscapes$\to$RobotCar.
(b) Comparison to state-of-the-art standard UDA methods on Cityscapes$\to$ACDC.
$\mathcal{SF}$ denotes a source-free adaptation approach.
}%
\label{tab:comp_robotcar_uda}
\end{table}


==> Tables/comp_sota.tex <==
\setlength{\floatsep}{10pt plus 0pt minus 5pt}
\setlength{\textfloatsep}{10pt plus 0pt minus 5pt}
\begin{table*}[t!]
\smallskip%
\centering%
\caption{Comparison with existing methods on Cityscapes $\to$ ACDC.
The results are reported in mIoU (\%) on the ACDC test set.}%
    % \vspace{-1mm}
% \vspace{-2mm}
\scalebox{0.62}{
\ra{1.3}%
% \normalsize
\begin{tabular}{@{}lcccccccccccccccccccr@{}}\toprule
\multirow{3}{*}{Method} & \multicolumn{19}{c}{ACDC IoU} \\
\cmidrule{2-21} & \rotatebox[origin=c]{90}{road} & \rotatebox[origin=c]{90}{sidew.} & \rotatebox[origin=c]{90}{build.} & \rotatebox[origin=c]{90}{wall} & \rotatebox[origin=c]{90}{fence} & \rotatebox[origin=c]{90}{pole} & \rotatebox[origin=c]{90}{light} & \rotatebox[origin=c]{90}{sign} & \rotatebox[origin=c]{90}{veget.} & \rotatebox[origin=c]{90}{terrain} & \rotatebox[origin=c]{90}{sky} & \rotatebox[origin=c]{90}{person} & \rotatebox[origin=c]{90}{rider} & \rotatebox[origin=c]{90}{car} & \rotatebox[origin=c]{90}{truck} & \rotatebox[origin=c]{90}{bus} & \rotatebox[origin=c]{90}{train} & \rotatebox[origin=c]{90}{motorc.} & \rotatebox[origin=c]{90}{bicycle} & \multicolumn{1}{c}{\phantom{00}\rotatebox[origin=c]{90}{\textbf{mean}}} \\ \midrule
Source model~\cite{xie2021segformer}  & 85.7 & 51.0 & 76.6 & 36.4 & 37.1 & 45.2 & 55.7 & 57.5 & 77.7 & 52.0 & 84.1 & 60.3 & 34.8 & 82.9 & 61.6 & 65.4 & 73.4 & 37.9 & 52.5 & 59.4 \\
HCL~\cite{huang2021model} & 86.4 & 53.5 & 78.5 & 38.8 & 38.1 & 48.0 & 57.8 & 58.9 & 78.1 & 52.4 & 85.1 & 61.7 & 37.1 & 83.7 & 64.1 & 66.6 & 74.5 & 39.1 & 53.3 & 60.8 \\
URMA~\cite{fleuret2021uncertainty} & 89.2 & 60.4 & 84.3 & 48.7 & 42.5 & 53.8 & 65.4 & 63.8 & 76.3 & 57.3 & 85.9 & 63.4 & 43.9 & 85.8 & \underline{68.8} & 73.2 & 82.8 & 46.3 & 48.4 & 65.3 \\
URMA + SimT~\cite{guo2022simt} & 90.0 & 65.7 & 80.6 & 46.0 & 41.7 & \underline{56.3} & 65.2 & 62.7 & 75.9 & 55.6 & 84.4 & 66.4 & \underline{46.6} & 85.4 & 68.4 & 72.3 & 80.0 & \underline{46.8} & 58.0 & 65.7 \\
% \midrule
CMA~\cite{bruggemann2023contrastive} & \textbf{94.0} & \textbf{75.2} & \textbf{88.6} & \underline{50.5} & \underline{45.5} & 54.9 & \underline{65.7} & \underline{64.2} & \textbf{87.1} & \textbf{61.3} & \underline{95.2} & \underline{67.0} & 45.2 & \underline{86.2} & 68.6 & \underline{76.6} & \textbf{83.9} & 43.3 & \underline{60.5} & \underline{69.1} \\
FREST (Ours) & \underline{93.3} & \underline{72.2} & \underline{88.3} & \textbf{52.4} & \textbf{46.6} & \textbf{58.6} & \textbf{66.2} & \textbf{66.1} & \underline{86.1} & \underline{58.6} & \textbf{95.3} & \textbf{69.9} & \textbf{49.2} & \textbf{89.1} & \textbf{75.1} & \textbf{79.4} & \underline{83.0} & \textbf{52.9} & \textbf{61.4}  & \textbf{70.7} \\
\bottomrule
\end{tabular}
}
% \vspace{-2.5mm}
% \vspace{-1mm}
\label{tab:acdc_sota}
\end{table*}


==> Tables/comp_study_classification.tex <==
\begin{table}[!t]
    \centering
    \renewcommand{\arraystretch}{1.0}
    \scalebox{1.0}{\begin{tabular}{lc}
    \toprule
    Possible Solution & mIoU \\
    \midrule
       Residual learning        &  62.8      \\
       Minimizing mutual information  &  65.6   \\
       Maximizing feature distance   &  66.5   \\
       Maximizing feature statistics   &   67.4   \\
       Feature classification (Ours)   & \textbf{68.6}       \\
     \bottomrule
    \end{tabular}}
    \caption{
    Analysis of possible solutions for adverse condition distancing loss.
    }
    \label{tab:abl_classifier}
    % \vspaceBottomTable
\end{table}

==> __misc__.tex <==
%!TEX root = ../main.tex

%%%%%%%%%% easy referencing
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\Sec}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\Tbl}[1]{Table~\ref{tab:#1}}
\newcommand{\Alg}[1]{Algorithm~\ref{algo:#1}}


% custom definition
\def\ie{\textit{i.e.}}
\def\eg{\textit{e.g.}}
\def\wrt{\textit{w.r.t.}}


% revision colors
\definecolor{brown}{rgb}{0.85, 0.15, 0.15}
\definecolor{purp}{rgb}{0.95, 0.16, 0.65}
\definecolor{purpc}{rgb}{0.95, 0.36, 0.65}
\definecolor{orange}{rgb}{0.9, 0.45, 0.0}
\definecolor{blue}{rgb}{0.0, 0.5, 1.0}
\definecolor{green}{rgb}{0, 0.8, 0}
\definecolor{lgreen}{rgb}{0.6, 0.8, 0}
\definecolor{red}{rgb}{0.8, 0, 0}
\definecolor{redd}{rgb}{0.9, 0, 0}
\definecolor{yellow}{rgb}{0.75, 0.56, 0}
\definecolor{darkblue}{rgb}{0.2, 0.2, 0.8}
\definecolor{brinkpink}{rgb}{0.98, 0.38, 0.5}
\definecolor{cadmiumred}{rgb}{0.89, 0.0, 0.13}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{dandelion}{rgb}{0.94, 0.88, 0.19}
\definecolor{bostonuniversityred}{rgb}{0.8, 0.0, 0.0}
\definecolor{brown(web)}{rgb}{0.65, 0.16, 0.16}
\definecolor{cornellred}{rgb}{0.7, 0.11, 0.11}
\definecolor{greend}{rgb}{0.0, 0.35, 0.0}


\newcommand{\redd}[1]{{\color{redd}{#1}}}
\newcommand{\greend}[1]{{\color{greend}{#1}}}
\newcommand{\yellowd}[1]{{\color{yellow}{#1}}}
% \newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcommand{\recap}[1]{{\color{blue}{#1}}}
\newcommand{\suha}[1]{{\color{darkblue}{#1}}}
\newcommand{\suhac}[1]{{\color{orange}{(#1)}}}
\newcommand{\sohyun}[1]{{\color{black}{#1}}}
\newcommand{\sohyunc}[1]{{\color{dandelion}{#1}}}
\newcommand{\ny}[1]{{\color{brown(web)}{#1}}}
\newcommand{\nyc}[1]{{\color{brown(web)}{(#1)}}}
\newcommand{\sy}[1]{{\color{cadmiumred}{#1}}}

% \newcommand{\recap}[1]{{\color{black}{#1}}}
% \newcommand{\suha}[1]{{\color{black}{#1}}}
% \newcommand{\suhac}[1]{{\color{black}{(#1)}}}
% \newcommand{\sohyun}[1]{{\color{black}{#1}}}
% \newcommand{\sohyunc}[1]{{\color{black}{#1}}}
% \newcommand{\ny}[1]{{\color{black}{#1}}}
% \newcommand{\nyc}[1]{{\color{black}{(#1)}}}
% \newcommand{\sy}[1]{{\color{black}{#1}}}


\newcommand{\supp}[1]{{\color{bostonuniversityred}{#1}}}

%\interfootnotelinepenalty=10000 % to force one-column footnote
\newcommand{\vspaceBottomFigure}{{\vspace{-3.5mm}}}
\newcommand{\vspaceBottomTable}{{\vspace{-3.0mm}}}
\newcommand{\firstparagraph}{\indent\indent}
%%%%%%%%%% small break paragraph
\newcommand{\smallbreakparagraph}[1]{\smallbreak \noindent \textbf{#1}}


%%%%%%%%%% Fig, Table, Eq. commands
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\tableref}[1]{Table~\ref{#1}}
% \newcommand{\eqref}[1]{Eq.~(\ref{#1})}


%%%%%%%%%% citations
\def\etal{\textit{et al.}}


%%%%%%%%%% math commands
\newcommand\mathopbelow[1]{\mathop{\operatorname{#1}}}

%%%%%%%%%% v and x marks
% tip: you need \usepackage{pifont}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}


%%%%%%%%%% table column colors
% tip: you need \usepackage{colortbl}
\definecolor{grey}{rgb}{0.9, 0.9, 0.9}
\newcommand{\ccol}{\cellcolor{grey}}

%%%%%%%%%% paper-specific commands
\DeclareMathOperator*{\argmin}{argmin} % no space, limits underneath in displays
\DeclareMathOperator*{\argmax}{argmax} % no space, limits underneath in displays
\newcommand{\itmini}{\textit{mini}}
\newcommand{\ittiered}{\textit{tiered}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\texts}{{\text{s}}}
\newcommand{\textq}{{\text{q}}}
\newcommand{\textk}{{\text{k}}}
\newcommand{\textS}{{\text{S}}}
\newcommand{\textL}{{\text{L}}}
\newcommand{\textT}{{\text{T}}}
\newcommand{\textP}{{\text{P}}}
\newcommand{\textPL}{{\text{PL}}}

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%%%%%%%%%% paper-specific commands (short arrow)
\newcommand{\veryshortarrow}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}
  
% Footnote url
% Make clickable footnote
\newcommand{\hyperfootnote}[1][]{\def\ArgI\hyperfootnoteRelay}
% relay to new command to make extra optional command possible
\newcommand\hyperfootnoteRelay[2][]{\href{#1#2}{\ArgI}\footnote{\href{#1#2}{#2}}}
% the first optional argument is now in \ArgI, the second is in #1

==> algorithm.tex <==

\begin{algorithm} [h!]
    % \fontsize{8}{10}\selectfont
    % \caption{: Training Our Framework}\label{alg:alg}
    \caption{: Training Algorithm of FREST}\label{alg:alg}
    \textbf{Input:} Condition strainer: $\psi_\textrm{strainer}$, Projection head: $\psi_\textrm{proj}$, $l^\textrm{th}$ layer of encoder: $\phi_{\textrm{enc}}^l$, Decoder: $\phi_{\textrm{dec}}$, Number of layers: $L$, Prediction: $P$, Pseudo Label: $\hat{Y}$, Input images: $\{x_\textrm{adv}$, $x_\textrm{norm}\}$
    
    \textbf{Output:} Optimized encoder $\phi_{\textrm{enc}}$ and decoder  $\phi_{\textrm{dec}}$.
    
    \begin{algorithmic}[1]
    
    \For{\{1, \dots , \# of training iterations\}}
        \State Sample mini-batch $\{ x_\textrm{adv}, x_\textrm{norm} \}$
        \For{\{{$l \longleftarrow 1$ to $L$}\}}
        % \State $\textbf{c}^0 \longleftarrow \textbf{f}^0$
        % \State  $\textbf{f}^{l} \longleftarrow \phi^l_{\textrm{enc}}(\textbf{f}^{l-1})$
        \State  $\textbf{c}_\textrm{adv}^{l} = \phi_{\textrm{enc}}^l(\textbf{c}_\textrm{adv}^{l-1})+\psi_\textrm{strainer}^l(\textbf{c}_\textrm{adv}^{l-1})$ 
        \State  $\textbf{c}_\textrm{norm}^{l} = \phi_{\textrm{enc}}^l(\textbf{c}_\textrm{norm}^{l-1})+\psi_\textrm{strainer}^l(\textbf{c}_\textrm{norm}^{l-1})$
        \EndFor
        \State $\mathcal{L}_\textrm{spec} = \mathcal{L}_{\textrm{spec}}(\psi_\textrm{proj}(\textbf{c}_\textrm{adv}), \psi_\textrm{proj}({\textbf{c}}_\textrm{norm}))$ \Comment{Eq.~(1)\&(2)}
        \State \textbf{Update} projection head $\psi_\textrm{proj} $ 
        \State $\mathcal{L}_\textrm{self} = \mathcal{L}_\textrm{self}(P_\textrm{adv},\hat{Y}_\textrm{adv})$ 
        % \State $\mathcal{L}_{\textrm{proj}} = \lambda_\textrm{spec}\mathcal{L}_{\textrm{spec}}$
        % \State \textbf{Update} projection head  $\psi_\textrm{proj}$ \textrm{with} $\mathcal{L}_{\textrm{proj}}$
        \State $\mathcal{L}_{\textrm{strainer}} = \lambda_\textrm{spec}\mathcal{L}_{\textrm{spec}} + \mathcal{L}_\textrm{self}$
        \State \textbf{Update} condition strainer $\psi_\textrm{strainer} $ \textrm{with} $\mathcal{L}_{\textrm{strainer}}$ \Comment{Step 1}
        % \State $\mathcal{L}_\textrm{dis}^0 = 0$
        \For{\{{$l \longleftarrow 1$ to $L$}\}}
        \State  $\textbf{f}_\textrm{adv}^{l} = \phi^l_{\textrm{enc}}(\textbf{f}_\textrm{adv}^{l-1})$
        \State  $\textbf{c}_\textrm{adv}^{l} = \phi_{\textrm{enc}}^l(\textbf{f}_\textrm{adv}^{l-1})+\psi_\textrm{strainer}^l(\textbf{f}_\textrm{adv}^{l-1})$ 
        % \State  $\textbf{c}_\textrm{norm}^{l} = \phi_{\textrm{enc}}^l(\textbf{c}_\textrm{norm}^{l-1})+\psi_\textrm{strainer}^l(\textbf{c}_\textrm{norm}^{l-1})$
        \State $\mathcal{L}_\textrm{dis}^l = -\mathcal{L}_\textrm{dis}^l(\textbf{f}_\textrm{adv}^l,\textbf{c}_\textrm{adv}^l)$ \Comment{Eq.~(4)}
        % \State $\mathcal{L}_\textrm{dis}^l = \mathcal{L}_\textrm{dis}^{l-1} + \mathcal{L}_\textrm{dis}^l(\textbf{f}_\textrm{adv}^l,\textbf{c}_\textrm{adv}^l)$
        \EndFor
        \State $\mathcal{L}_\textrm{self} = \mathcal{L}_\textrm{self}(P_\textrm{adv},\hat{Y}_\textrm{adv})$ 
        \State $\mathcal{L}_\textrm{resto} = \mathcal{L}_\textrm{resto}(\psi_\textrm{proj}(\textbf{f}_\textrm{adv}),\psi_\textrm{proj}({\textbf{c}}_\textrm{norm}))$ \Comment{Eq.~(3)}
        \State $\mathcal{L}_{\textrm{total}} =
        \mathcal{L}_\textrm{self} + \lambda_\textrm{ent}\mathcal{L}_\textrm{ent} + \mathcal{L}_\textrm{resto} + \lambda_\textrm{dis}\sum_{l=1}\mathcal{L}_\textrm{dis}^l$
        \State \textbf{Update} $\phi_{\textrm{enc}}$ and $\phi_{\textrm{dec}}$ of the model \textrm{with} $\mathcal{L}_{\textrm{total}}$ 
    \Comment{Step 2}
    \EndFor
    
    \end{algorithmic}
\end{algorithm}\label{algo}

% \begin{algorithm} [t!]
%     \caption{Training Our Framework}\label{alg:alg}
%     \textbf{Input:} Condition filter: $F(\cdot)$, Condition amplifier: $A(\cdot)$, Segmentation network: $S(\cdot)$, Number of layers: $L$, Prediction: $P$, Pseudo Label: $\hat{Y}$, Input images: $x_\textrm{adv}$, $x_\textrm{norm}$
    
%     \textbf{Output:} Optimized segmentation network $S(\cdot)$.
    
%     \begin{algorithmic}[1]
    
%     \For{\textcolor{blue}{Each training iteration}}
%         \State \textcolor{blue}{Sample mini-batch: $\{ x_\textrm{adv}, x_\textrm{norm} \}$}
%         \For{\textcolor{blue}{Each layer $l = 1$ to $L$}}
%         \State \textcolor{blue}{Feature extraction: $\textbf{f}^{l} = \phi^l_{\textrm{enc}}(\textbf{f}^{l-1})$}
%         \State \textcolor{blue}{Feature update: $\textbf{c}^{l} = \phi^l_{\textrm{enc}}(\textbf{c}^{l-1})+A^l(\textbf{c}^{l-1})$}
%         \EndFor
%         \State \textcolor{blue}{Condition Filter Loss: $\mathcal{L}_{\textrm{filter}} = \lambda_\textrm{spec}\mathcal{L}_{\textrm{spec}}(\textbf{c}_\textrm{adv}^{L}, \textbf{c}_\textrm{norm}^{L})$}
%         \State \textcolor{blue}{Update the condition filter $F$}
%         \State \textcolor{blue}{Condition amplifier Loss: $\mathcal{L}_{\textrm{amplifier}} = \lambda_\textrm{spec}\mathcal{L}_{\textrm{spec}}(\textbf{c}_\textrm{adv}^{L}, \textbf{c}_\textrm{norm}^{L}) + \mathcal{L}_\textrm{st}(P_\textrm{adv},\hat{Y}_\textrm{adv})$}
%         \State \textcolor{blue}{Update the condition amplifier $A$}
%         \For{\textcolor{blue}{Each layer $l = 1$ to $L$}}
%         \State \textcolor{blue}{Disentanglement Loss: $\mathcal{L}_\textrm{dis}^l = \mathcal{L}_\textrm{dis}^{l-1} + \mathcal{L}_\textrm{dis}^l(\textbf{f}_\textrm{adv}^l,\textbf{c}_\textrm{adv}^l)$}
%         \EndFor
%         \State \textcolor{blue}{Total Loss: $\mathcal{L}_{\textrm{total}} =
%         \mathcal{L}_\textrm{st}(P_\textrm{adv},\hat{Y}_\textrm{adv}) + \lambda_\textrm{ent}\mathcal{L}_\textrm{ent}(P_\textrm{adv}) + \lambda_\textrm{ng}\mathcal{L}_\textrm{ng}(\textbf{f}_\textrm{adv}^{L},\textbf{c}_\textrm{norm}^{L}) + \mathcal{L}_\textrm{dis}^L$}
%         \State \textcolor{blue}{Update the segmentation network $S$}
%     \EndFor
    
%     \end{algorithmic}
% \end{algorithm}
